SetLexSem Challenge: Using Set Operations to Evaluate the Lexical and Semantic Robustness of Language Models

Set theory is foundational to mathematics and, when sets are finite, to reasoning about the world. An intelligent system should perform set operations consistently, regardless of superficial variations in the operands. Initially designed for semantically-oriented NLP tasks, large language models (LLMs) are now being evaluated on algorithmic tasks. Because sets are comprised of arbitrary symbols (e.g. numbers, words), they provide an opportunity to test, systematically, the invariance of LLMs' algorithmic abilities under simple lexical or semantic variations. To this end, we present the SetLexSem Challenge, a synthetic benchmark that evaluates the performance of LLMs on set operations. SetLexSem assesses the robustness of LLMs' instruction-following abilities under various conditions, focusing on the set operations and the nature and construction of the set members. Evaluating seven LLMs with SetLexSem, we find that they exhibit poor robustness to variation in both operation and operands. We show -- via the framework's systematic sampling of set members along lexical and semantic dimensions -- that LLMs are not only not robust to variation along these dimensions but demonstrate unique failure modes in particular, easy-to-create semantic groupings of "deceptive" sets. We find that rigorously measuring language model robustness to variation in frequency and length is challenging and present an analysis that measures them independently. The code for reproducing the results of this paper, and for generating the SetLexSem Challenge dataset, is available at \href{https://github.com/amazon-science/SetLexSem-Challenge}{https://github.com/amazon-science/SetLexSem-Challenge}.

==> bibliography.tex <==
\begin{thebibliography}{40}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Vaswani et~al.(2017)Vaswani, Shazeer, Parmar, Uszkoreit, Jones, Gomez,
  Kaiser, and Polosukhin]{NIPS2017_3f5ee243}
Ashish Vaswani, Noam Shazeer, Niki Parmar, Jakob Uszkoreit, Llion Jones,
  Aidan~N Gomez, \L~ukasz Kaiser, and Illia Polosukhin.
\newblock
  \href{https://proceedings.neurips.cc/paper_files/paper/2017/file/3f5ee243547dee91fbd053c1c4a845aa-Paper.pdf}{Attention
  is All you Need}.
\newblock In \emph{Advances in Neural Information Processing Systems}, 2017.

\bibitem[Devlin et~al.(2019)Devlin, Chang, Lee, and
  Toutanova]{devlin-etal-2019-bert}
Jacob Devlin, Ming-Wei Chang, Kenton Lee, and Kristina Toutanova.
\newblock \href{https://aclanthology.org/N19-1423}{{BERT}: Pre-training of Deep
  Bidirectional Transformers for Language Understanding}.
\newblock In \emph{Proceedings of the North {A}merican Chapter of the
  Association for Computational Linguistics}, 2019.

\bibitem[Wang et~al.(2018)Wang, Singh, Michael, Hill, Levy, and
  Bowman]{wang-etal-2018-glue}
Alex Wang, Amanpreet Singh, Julian Michael, Felix Hill, Omer Levy, and Samuel
  Bowman.
\newblock \href{https://aclanthology.org/W18-5446}{{GLUE}: A Multi-Task
  Benchmark and Analysis Platform for Natural Language Understanding}.
\newblock In \emph{Proceedings of the {EMNLP} Workshop {B}lackbox{NLP}:
  Analyzing and Interpreting Neural Networks for {NLP}}, 2018.

\bibitem[Rajpurkar et~al.(2018)Rajpurkar, Jia, and
  Liang]{rajpurkar-etal-2018-know}
Pranav Rajpurkar, Robin Jia, and Percy Liang.
\newblock \href{https://aclanthology.org/P18-2124}{Know What You Don{'}t Know:
  Unanswerable Questions for {SQ}u{AD}}.
\newblock In \emph{Association for Computational Linguistics}, 2018.

\bibitem[Ouyang et~al.(2022)Ouyang, Wu, Jiang, Almeida, Wainwright, Mishkin,
  Zhang, Agarwal, Slama, Ray, et~al.]{ouyang2022training}
Long Ouyang, Jeffrey Wu, Xu~Jiang, Diogo Almeida, Carroll Wainwright, Pamela
  Mishkin, Chong Zhang, Sandhini Agarwal, Katarina Slama, Alex Ray, et~al.
\newblock
  \href{https://proceedings.neurips.cc/paper_files/paper/2022/hash/b1efde53be364a73914f58805a001731-Abstract-Conference.html}{Training
  language models to follow instructions with human feedback}.
\newblock \emph{Advances in Neural Information Processing Systems}, 2022.

\bibitem[Cobbe et~al.(2021)Cobbe, Kosaraju, Bavarian, Chen, Jun, Kaiser,
  Plappert, Tworek, Hilton, Nakano, et~al.]{cobbe2021training}
Karl Cobbe, Vineet Kosaraju, Mohammad Bavarian, Mark Chen, Heewoo Jun, Lukasz
  Kaiser, Matthias Plappert, Jerry Tworek, Jacob Hilton, Reiichiro Nakano,
  et~al.
\newblock \href{https://arxiv.org/abs/2110.14168}{Training verifiers to solve
  math word problems}.
\newblock \emph{arXiv:2110.14168}, 2021.

\bibitem[Hendrycks et~al.(2021{\natexlab{a}})Hendrycks, Burns, Kadavath, Arora,
  Basart, Tang, Song, and Steinhardt]{hendrycks2021measuring}
Dan Hendrycks, Collin Burns, Saurav Kadavath, Akul Arora, Steven Basart, Eric
  Tang, Dawn Song, and Jacob Steinhardt.
\newblock \href{https://openreview.net/forum?id=7Bywt2mQsCe}{Measuring
  Mathematical Problem Solving With the {MATH} Dataset}.
\newblock In \emph{Advances in Neural Information Processing Systems},
  2021{\natexlab{a}}.

\bibitem[Dua et~al.(2019)Dua, Wang, Dasigi, Stanovsky, Singh, and
  Gardner]{dua-etal-2019-drop}
Dheeru Dua, Yizhong Wang, Pradeep Dasigi, Gabriel Stanovsky, Sameer Singh, and
  Matt Gardner.
\newblock \href{https://aclanthology.org/N19-1246}{{DROP}: A Reading
  Comprehension Benchmark Requiring Discrete Reasoning Over Paragraphs}.
\newblock In \emph{Conference of the North {A}merican Chapter of the
  Association for Computational Linguistics}, 2019.

\bibitem[Chen et~al.(2021)Chen, Tworek, Jun, Yuan, Pinto, Kaplan, Edwards,
  Burda, Joseph, Brockman, et~al.]{chen2021evaluating}
Mark Chen, Jerry Tworek, Heewoo Jun, Qiming Yuan, Henrique Ponde de~Oliveira
  Pinto, Jared Kaplan, Harri Edwards, Yuri Burda, Nicholas Joseph, Greg
  Brockman, et~al.
\newblock \href{https://arxiv.org/abs/2107.03374}{Evaluating large language
  models trained on code}.
\newblock \emph{arXiv:2107.03374}, 2021.

\bibitem[Li and Flanigan(2024)]{Li_Flanigan_2024}
Changmao Li and Jeffrey Flanigan.
\newblock Task contamination: Language models may not be few-shot anymore.
\newblock \emph{Proceedings of the AAAI Conference on Artificial Intelligence},
  38\penalty0 (16):\penalty0 18471--18480, Mar. 2024.
\newblock \doi{10.1609/aaai.v38i16.29808}.
\newblock URL \url{https://ojs.aaai.org/index.php/AAAI/article/view/29808}.

\bibitem[Zhang et~al.(2024)Zhang, Klyman, Mai, Levine, Zhang, Bommasani, and
  Liang]{zhang2024language}
Andy~K Zhang, Kevin Klyman, Yifan Mai, Yoav Levine, Yian Zhang, Rishi
  Bommasani, and Percy Liang.
\newblock Language model developers should report train-test overlap.
\newblock \emph{arXiv preprint arXiv:2410.08385}, 2024.

\bibitem[Kahneman(2011)]{kahneman2011thinking}
Daniel Kahneman.
\newblock \emph{Thinking, fast and slow}.
\newblock macmillan, 2011.

\bibitem[Zheng and Zhan(2023)]{zheng2023chatgpt}
Haoyi Zheng and Huichun Zhan.
\newblock
  \href{https://www.amjmed.com/article/S0002-9343(23)00159-6/fulltext}{ChatGPT
  in scientific writing: a cautionary tale}.
\newblock \emph{The American Journal of Medicine}, 136\penalty0 (8):\penalty0
  725--726, 2023.

\bibitem[Lin et~al.(2021)Lin, Jaech, Li, Gormley, and
  Eisner]{lin2020limitations}
Chu-Cheng Lin, Aaron Jaech, Xin Li, Matthew~R. Gormley, and Jason Eisner.
\newblock \href{https://aclanthology.org/2021.naacl-main.405}{Limitations of
  Autoregressive Models and Their Alternatives}.
\newblock In \emph{Conference of the North American Chapter of the Association
  for Computational Linguistics}, 2021.

\bibitem[Prystawski et~al.(2023)Prystawski, Li, and Goodman]{prystawski2023why}
Ben Prystawski, Michael~Y. Li, and Noah Goodman.
\newblock \href{https://openreview.net/forum?id=rcXXNFVlEn}{Why think step by
  step? Reasoning emerges from the locality of experience}.
\newblock In \emph{Advances in Neural Information Processing Systems}, 2023.

\bibitem[Welleck et~al.(2022)Welleck, West, Cao, and Choi]{welleck2022symbolic}
Sean Welleck, Peter West, Jize Cao, and Yejin Choi.
\newblock \href{https://arxiv.org/abs/2109.13986}{Symbolic brittleness in
  sequence models: on systematic generalization in symbolic mathematics}.
\newblock In \emph{Proceedings of the AAAI Conference on Artificial
  Intelligence}, 2022.

\bibitem[Geirhos et~al.(2020)Geirhos, Jacobsen, Michaelis, Zemel, Brendel,
  Bethge, and Wichmann]{geirhos2020shortcut}
Robert Geirhos, J{\"o}rn-Henrik Jacobsen, Claudio Michaelis, Richard Zemel,
  Wieland Brendel, Matthias Bethge, and Felix~A Wichmann.
\newblock \href{https://www.nature.com/articles/s42256-020-00257-z}{Shortcut
  learning in deep neural networks}.
\newblock \emph{Nature Machine Intelligence}, 2\penalty0 (11):\penalty0
  665--673, 2020.

\bibitem[Bogin et~al.(2022)Bogin, Gupta, and Berant]{bogin2022unobserved}
Ben Bogin, Shivanshu Gupta, and Jonathan Berant.
\newblock \href{https://aclanthology.org/2022.emnlp-main.175}{Unobserved Local
  Structures Make Compositional Generalization Hard}.
\newblock In \emph{Conference on Empirical Methods in Natural Language
  Processing}, 2022.

\bibitem[Sakaguchi et~al.(2021)Sakaguchi, Bras, Bhagavatula, and
  Choi]{10.1145/3474381}
Keisuke Sakaguchi, Ronan~Le Bras, Chandra Bhagavatula, and Yejin Choi.
\newblock \href{https://doi.org/10.1145/3474381}{WinoGrande: an adversarial
  winograd schema challenge at scale}.
\newblock \emph{Communications of the ACM}, 64\penalty0 (9):\penalty0 99–106,
  Aug 2021.

\bibitem[Hendrycks et~al.(2021{\natexlab{b}})Hendrycks, Burns, Basart, Zou,
  Mazeika, Song, and Steinhardt]{hendrycks2021measuringMMMLU}
Dan Hendrycks, Collin Burns, Steven Basart, Andy Zou, Mantas Mazeika, Dawn
  Song, and Jacob Steinhardt.
\newblock \href{https://openreview.net/forum?id=d7KBjmI3GmQ}{Measuring Massive
  Multitask Language Understanding}.
\newblock In \emph{International Conference on Learning Representations},
  2021{\natexlab{b}}.

\bibitem[Srivastava et~al.(2023)]{srivastava2022beyond}
Aarohi Srivastava et~al.
\newblock \href{https://openreview.net/forum?id=uyTL5Bvosj}{Beyond the
  Imitation Game: Quantifying and extrapolating the capabilities of language
  models}.
\newblock \emph{Transactions on Machine Learning Research}, 2023.

\bibitem[Suzgun et~al.(2023)Suzgun, Scales, Sch{\"a}rli, Gehrmann, Tay, Chung,
  Chowdhery, Le, Chi, Zhou, and Wei]{suzgun-etal-2023-challenging}
Mirac Suzgun, Nathan Scales, Nathanael Sch{\"a}rli, Sebastian Gehrmann, Yi~Tay,
  Hyung~Won Chung, Aakanksha Chowdhery, Quoc Le, Ed~Chi, Denny Zhou, and Jason
  Wei.
\newblock \href{https://aclanthology.org/2023.findings-acl.824}{Challenging
  {BIG}-Bench Tasks and Whether Chain-of-Thought Can Solve Them}.
\newblock In \emph{Findings of the Association for Computational Linguistics},
  2023.

\bibitem[Basmov et~al.(2024)Basmov, Goldberg, and Tsarfaty]{basmov2024llms}
Victoria Basmov, Yoav Goldberg, and Reut Tsarfaty.
\newblock \href{https://arxiv.org/abs/2404.06283}{LLMs' Reading Comprehension
  Is Affected by Parametric Knowledge and Struggles with Hypothetical
  Statements}.
\newblock \emph{arXiv:2404.06283}, 2024.

\bibitem[Razeghi et~al.(2022)Razeghi, Logan~IV, Gardner, and
  Singh]{razeghi-etal-2022-impact}
Yasaman Razeghi, Robert~L Logan~IV, Matt Gardner, and Sameer Singh.
\newblock \href{https://aclanthology.org/2022.findings-emnlp.59}{Impact of
  Pretraining Term Frequencies on Few-Shot Numerical Reasoning}.
\newblock In \emph{Findings of the Association for Computational Linguistics:
  EMNLP 2022}, 2022.

\bibitem[Dziri et~al.(2023)Dziri, Lu, Sclar, Li, Jiang, Lin, Welleck, West,
  Bhagavatula, Bras, Hwang, Sanyal, Ren, Ettinger, Harchaoui, and
  Choi]{dziri2023faith}
Nouha Dziri, Ximing Lu, Melanie Sclar, Xiang~Lorraine Li, Liwei Jiang,
  Bill~Yuchen Lin, Sean Welleck, Peter West, Chandra Bhagavatula, Ronan~Le
  Bras, Jena~D. Hwang, Soumya Sanyal, Xiang Ren, Allyson Ettinger, Zaid
  Harchaoui, and Yejin Choi.
\newblock \href{https://openreview.net/forum?id=Fkckkr3ya8}{Faith and Fate:
  Limits of Transformers on Compositionality}.
\newblock In \emph{Thirty-seventh Conference on Neural Information Processing
  Systems}, 2023.

\bibitem[Anil et~al.(2022)Anil, Wu, Andreassen, Lewkowycz, Misra, Ramasesh,
  Slone, Gur-Ari, Dyer, and Neyshabur]{NEURIPS2022_fb7451e4}
Cem Anil, Yuhuai Wu, Anders Andreassen, Aitor Lewkowycz, Vedant Misra, Vinay
  Ramasesh, Ambrose Slone, Guy Gur-Ari, Ethan Dyer, and Behnam Neyshabur.
\newblock
  \href{https://proceedings.neurips.cc/paper_files/paper/2022/file/fb7451e43f9c1c35b774bcfad7a5714b-Paper-Conference.pdf}{Exploring
  Length Generalization in Large Language Models}.
\newblock In \emph{Advances in Neural Information Processing Systems}, 2022.

\bibitem[Bueno et~al.(2022)Bueno, Gemmell, Dalton, Lotufo, and
  Nogueira]{bueno2022induced}
Mirelle~Candida Bueno, Carlos Gemmell, Jeff Dalton, Roberto Lotufo, and Rodrigo
  Nogueira.
\newblock \href{https://aclanthology.org/2022.mathnlp-1.3}{Induced Natural
  Language Rationales and Interleaved Markup Tokens Enable Extrapolation in
  Large Language Models}.
\newblock In \emph{Proceedings of the 1st Workshop on Mathematical Natural
  Language Processing (MathNLP)}, 2022.

\bibitem[Schwarzschild et~al.(2021)Schwarzschild, Borgnia, Gupta, Huang,
  Vishkin, Goldblum, and Goldstein]{NEURIPS2021_3501672e}
Avi Schwarzschild, Eitan Borgnia, Arjun Gupta, Furong Huang, Uzi Vishkin, Micah
  Goldblum, and Tom Goldstein.
\newblock
  \href{https://proceedings.neurips.cc/paper_files/paper/2021/file/3501672ebc68a5524629080e3ef60aef-Paper.pdf}{Can
  You Learn an Algorithm? Generalizing from Easy to Hard Problems with
  Recurrent Networks}.
\newblock In \emph{Advances in Neural Information Processing Systems}, 2021.

\bibitem[Bansal et~al.(2022)Bansal, Schwarzschild, Borgnia, Emam, Huang,
  Goldblum, and Goldstein]{NEURIPS2022_7f70331d}
Arpit Bansal, Avi Schwarzschild, Eitan Borgnia, Zeyad Emam, Furong Huang, Micah
  Goldblum, and Tom Goldstein.
\newblock
  \href{https://proceedings.neurips.cc/paper_files/paper/2022/file/7f70331dbe58ad59d83941dfa7d975aa-Paper-Conference.pdf}{End-to-end
  Algorithm Synthesis with Recurrent Networks: Extrapolation without
  Overthinking}.
\newblock In \emph{Advances in Neural Information Processing Systems}, 2022.

\bibitem[Brown et~al.(2020)Brown, Mann, Ryder, Subbiah, Kaplan, Dhariwal,
  Neelakantan, Shyam, Sastry, Askell, et~al.]{brown2020language}
Tom Brown, Benjamin Mann, Nick Ryder, Melanie Subbiah, Jared~D Kaplan, Prafulla
  Dhariwal, Arvind Neelakantan, Pranav Shyam, Girish Sastry, Amanda Askell,
  et~al.
\newblock \href{https://arxiv.org/abs/2005.14165}{Language models are few-shot
  learners}.
\newblock \emph{Advances in Neural Information Processing Systems}, 2020.

\bibitem[Levy et~al.(2022)Levy, Bogin, and Berant]{levy2022diverse}
Itay Levy, Ben Bogin, and Jonathan Berant.
\newblock \href{https://aclanthology.org/2023.acl-long.78/}{Diverse
  demonstrations improve in-context compositional generalization}.
\newblock \emph{arXiv:2212.06800}, 2022.

\bibitem[Zhou et~al.(2022)Zhou, Nova, Larochelle, Courville, Neyshabur, and
  Sedghi]{zhou2022teaching}
Hattie Zhou, Azade Nova, Hugo Larochelle, Aaron Courville, Behnam Neyshabur,
  and Hanie Sedghi.
\newblock \href{https://arxiv.org/abs/2211.09066}{Teaching algorithmic
  reasoning via in-context learning}.
\newblock \emph{arXiv:2211.09066}, 2022.

\bibitem[Wei et~al.(2022)Wei, Wang, Schuurmans, Bosma, Xia, Chi, Le, Zhou,
  et~al.]{wei2022chain}
Jason Wei, Xuezhi Wang, Dale Schuurmans, Maarten Bosma, Fei Xia, Ed~Chi, Quoc~V
  Le, Denny Zhou, et~al.
\newblock
  \href{https://proceedings.neurips.cc/paper_files/paper/2022/hash/9d5609613524ecf4f15af0f7b31abca4-Abstract-Conference.html}{Chain-of-thought
  prompting elicits reasoning in large language models}.
\newblock \emph{Advances in Neural Information Processing Systems}, 2022.

\bibitem[Qin et~al.(2023)Qin, Zhang, Zhang, Chen, Yasunaga, and
  Yang]{qin2023chatgpt}
Chengwei Qin, Aston Zhang, Zhuosheng Zhang, Jiaao Chen, Michihiro Yasunaga, and
  Diyi Yang.
\newblock \href{https://arxiv.org/abs/2302.06476}{Is ChatGPT a general-purpose
  natural language processing task solver?}
\newblock \emph{arXiv:2302.06476}, 2023.

\bibitem[Merrill and Sabharwal(2023)]{merrill2023expresssive}
William Merrill and Ashish Sabharwal.
\newblock \href{https://arxiv.org/abs/2310.07923}{The expresssive power of
  transformers with chain of thought}.
\newblock \emph{arXiv:2310.07923}, 2023.

\bibitem[Anthropic(2024)]{Prompt_engineering}
Anthropic.
\newblock
  \href{https://docs.anthropic.com/claude/docs/prompt-engineering}{Performance
  Enhancement - Use XML Tags}, 2024.

\bibitem[Bird and Loper(2004)]{bird-loper-2004-nltk}
Steven Bird and Edward Loper.
\newblock \href{https://aclanthology.org/P04-3031}{{NLTK}: The Natural Language
  Toolkit}.
\newblock In \emph{Proceedings of the Association of Computational
  Linguistics}, 2004.

\bibitem[Google(2024)]{Google_Ngram_Viewer_2024}
Google.
\newblock
  \href{https://en.wikipedia.org/w/index.php?title=Google_Ngram_Viewer&oldid=1208322096}{Google~NGram~Viewer},
  February 2024.
\newblock Page Version ID: 1208322096.

\bibitem[Miller(1995)]{10.1145/219717.219748}
George~A. Miller.
\newblock \href{https://doi.org/10.1145/219717.219748}{WordNet: a lexical
  database for English}.
\newblock \emph{Communications of the ACM}, 38\penalty0 (11):\penalty0 39–41,
  nov 1995.
\newblock ISSN 0001-0782.

\bibitem[Schaeffer et~al.(2024)Schaeffer, Miranda, and
  Koyejo]{schaeffer2024emergent}
Rylan Schaeffer, Brando Miranda, and Sanmi Koyejo.
\newblock Are emergent abilities of large language models a mirage?
\newblock \emph{Advances in Neural Information Processing Systems}, 36, 2024.

\end{thebibliography}

